End-to-End Weak Supervision

Aggregating multiple sources of weak supervision (WS) can ease the data-labeling bottleneck prevalent in many machine learning applications, by replacing the tedious manual collection of ground truth labels. Current state of the art approaches that do not use any labeled training data, however, require two separate modeling steps: Learning a probabilistic latent variable model based on the WS sources -- making assumptions that rarely hold in practice -- followed by downstream model training. Importantly, the first step of modeling does not consider the performance of the downstream model. To address these caveats we propose an end-to-end approach for directly learning the downstream model by maximizing its agreement with probabilistic labels generated by reparameterizing previous probabilistic posteriors with a neural network. Our results show improved performance over prior work in terms of end model performance on downstream test sets, as well as in terms of improved robustness to dependencies among weak supervision sources.

==> sections/9999checklist.tex <==
\newpage
\section*{Checklist}
\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{See section \ref{sec:practicalAspects}}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{Potential negative societal impacts are not specific to our new method, but to the overall studied area of (multi-source) weak supervision. We provide a brief discussion of this in Appendix \ref{sec:broaderImpact}.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{See supplementary code and instructions therein (README.md)}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{Dataset details are in section \ref{Experiments} and see section \ref{sec:implDetails} in the appendix for hyperparameter details, as well as appendix \ref{sec:crowdsourcingAppendix} and \ref{sec:robustnessAppendix} for training \& baseline setup details specific to the crowdsourcing and model robustness experiments, respectively.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{For the main experiments/benchmarking seven random seeds were used, for all other experiments at least five random seeds were used (and the standard deviations across the seeds are always reported).}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerNo{}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{See dataset paragraph in section \ref{Experiments}, and README.md in the data- and LF- set link in the supplementary material (\url{https://drive.google.com/drive/u/2/folders/1v7IzA3Ab5zDEsRpLBWmJnXo5841tSOlh})}
  \item Did you mention the license of the assets?
    \answerNo{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{Yes, instructions to download the main datasets and LF sets (including the newly introduced sets) used are included in the source code README.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{All data was public and no data agreements were needed.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerYes{We state that all datasets were publicly released, commonly used benchmark datasets, none of which contain sensitive personally identifiable information.}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{We used publicly released crowdsourcing benchmark data but did not conduct crowdsourcing exercises}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

==> tables/labelMeFULL.tex <==
% \begin{table}[htp]
% \caption{Test accuracy scores on the crowsourced, multi-class LabelMe image classification dataset. MV refers to the majority vote. DoctorNet was proposed in \cite{doctorNet}, Crowd Layer in \cite{rodrigues2018deep}, MaxMIG in \cite{MaxMIG}. Our try to reproduce \cite{MaxMIG} resulted in an accuracy of 83.90 $\pm$ 0.34 only.}
% \begin{center}
% \begin{tabular}{llllllllll}
% \toprule
%     Model &
%         MV &
%         DoctorNet & 
%         Crowd Layer &
%         MaxMIG &
%         Snorkel &
%         Snorkel+MIG &
%         E2E & % $\mathrm{E2E}$ &
%         E2E+MIG % $\mathrm{E2E+MIG}$
%         \\
%     \midrule\midrule
%     Accuracy & 
%         $80.41 \pm 0.6$  & 
%         $80.56 \pm 0.6$  & 
%         $83.65 \pm 0.5$  &
%         $86.42 \pm 0.4$  &
%         79.76 $\pm$ 1.3  &
%         84.03 $\pm$ 0.6  &
%         80.99 $\pm$ 0.5  &
%         86.21 $\pm$ 0.5  
          
%     \\ 
%     \bottomrule
% \end{tabular}
% \end{center}
% \label{table:distinguishers}
% \end{table}
\begin{table}[htp]
\caption{Test accuracy scores on the crowd-sourced, multi-class LabelMe image classification dataset. Experiments were conducted over seven random seeds with a learning rate of 1e-4 and 50 epochs. The reported scores are the ones with best validation set (of size 200) accuracy for a L2 weight decay $\in \{$ 7e-7, 1e-4 $\}$.
}
\begin{center}
\begin{tabular}{llllllllll}
\toprule
    Model & Accuracy \\ 
    \midrule
        Majority vote        & $79.23 \pm 0.49$\\  
        MBEM \cite{khetan2017learning} & $76.84 \pm 0.37$ \\
        DoctorNet \cite{doctorNet} & $81.31 \pm 0.44$\\ 
        CrowdLayer \cite{rodrigues2018deep} & $82.83 \pm 0.44$\\ 
        AggNet \cite{aggNet} & $84.35 \pm 0.39$ \\
        MaxMIG \cite{MaxMIG} & \second{85.45 $\pm$ 0.98}\\ 
        Snorkel+CE & $82.89 \pm 0.72$\\ 
        E2E+CE & $82.46 \pm 0.75$\\             % $\mathrm{E2E}$ &
        Snorkel+MIG & $85.15 \pm 0.76$\\ 
        E2E+MIG & \first{86.36 $\pm$ 0.31}\\     % $\mathrm{E2E+MIG}$
    \bottomrule
    \label{tab:labelMeFull}
\end{tabular}
\end{center}
\end{table}
